LiveLongBench: Tackling Long-Context Understanding for Spoken Texts from Live Streams

Long-context understanding poses significant challenges in natural language processing, particularly for real-world dialogues characterized by speech-based elements, high redundancy, and uneven information density. Although large language models (LLMs) achieve impressive results on existing benchmarks, these datasets fail to reflect the complexities of such texts, limiting their applicability to practical scenarios. To bridge this gap, we construct the first spoken long-text dataset, derived from live streams, designed to reflect the redundancy-rich and conversational nature of real-world scenarios. We construct tasks in three categories: retrieval-dependent, reasoning-dependent, and hybrid. We then evaluate both popular LLMs and specialized methods to assess their ability to understand long-contexts in these tasks. Our results show that current methods exhibit strong task-specific preferences and perform poorly on highly redundant inputs, with no single method consistently outperforming others. We propose a new baseline that better handles redundancy in spoken text and achieves strong performance across tasks. Our findings highlight key limitations of current methods and suggest future directions for improving long-context understanding. Finally, our benchmark fills a gap in evaluating long-context spoken language understanding and provides a practical foundation for developing real-world e-commerce systems. The code and benchmark are available at https://github.com/Yarayx/livelongbench.

==> methods2.tex <==
% n\section{LongLEcTE: A Long-Context Benchmark in Live Streaming E-commerce}
\usepackage{xcolor}
\section{LiveLongBench}
% \subsection{Design Principles}
\subsection{Basic Challenges}
We aim to construct a dataset that captures the real-world challenges associated with long-context processing, particularly the issues of \emph{informal language} and \emph{high redundancy}. 
Live-streaming, with its spontaneous conversational style and repetitive content, exemplifies these challenges through numerous real-world instances, making it an ideal domain for studying long spoken text understanding.
% First, live commerce often involves conversational speech that includes fillers, incomplete sentences, and colloquial expressions, all of which contribute to the informality of the language. Second, in live commerce settings, presenters frequently repeat information to emphasize key product features, leading to redundancy in the discourse that can hinder effective understanding and processing of long contexts. 

\begin{figure}[!t]
\begin{tcolorbox}
\small
$\vartriangleright$ \textbf{Syntactic Reduction:} \\
\emph{``Big scarf The discount office.''}\\~\textcolor{orange}{Verbless}\\
\emph{``This place, the focus of our vision.''}\\~\textcolor{orange}{Right-Dislocation}\\
\\
$\vartriangleright$ \textbf{Topic Drift:} \\
\emph{``This handbag is made of genuine leather and comes in three colors. I bought one for my sister last week... Oh, by the way, did you see the movie I talked about yesterday?''}
~\textcolor{orange}{From product details to unrelated personal topics}
\end{tcolorbox}
\end{figure}

\paragraph{Informal Language.}
Live-streaming e-commerce data often involves conversational speech, contributing to the informality of the language. Unlike formal text, live-stream content typically consists of short, fragmented utterances, leading to a high occurrence of syntactic reduction (accounting for \textcolor{blue}{XX\%} of the dataset). Additionally, interactive conversations with viewers frequently introduce topic drift (observed in  \textcolor{blue}{XX\%} of the data), where discussions shift abruptly, making it difficult for models to maintain contextual coherence. These characteristics significantly increase the complexity of document understanding compared to well-structured formal text.

\paragraph{High Redundancy.}
Live-stream transcripts contain a substantial amount of filler words (comprising \textcolor{blue}{XX\%} of the dataset). To emphasize key product features, presenters often include repetitive content (accounting for \textcolor{blue}{XX\%}), reiterating the same information multiple times. Furthermore, interactive dialogues introduce additional non-informative tokens (representing \textcolor{blue}{XX\%} of the text), which inflate the overall length while lowering the density of useful information. This high redundancy poses challenges for long-context processing, requiring models to efficiently filter out noise while retaining essential details.

\begin{figure}[!t]
\begin{tcolorbox}
\small
$\vartriangleright$ \textbf{Filler Words:} \\
\emph{``Um, okay, so, yeah, you know, like, I mean, actually, basically...''}\\
\\
$\vartriangleright$ \textbf{Repetitive Content:} \\
\emph{``This bag is beautiful, really beautiful, so beautiful! I mean, it’s just beautiful!''}\\
\\
$\vartriangleright$ \textbf{Non-informative Tokens:} \\
\emph{``This is really nice, you know? It’s just so good. Like, really good, you know what I mean?''}\\
\end{tcolorbox}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/english_wordcloud.pdf}
    \caption{Wordcloud}
    \label{fig:Wordcloud}
\end{figure}

% In long-context discourse, it is common to encounter instances where the narrative experiences abrupt shifts in topic, leading to interruptions in the original line of discussion. This phenomenon—often referred to as topic drift—manifests when a speaker, while initially focused on describing a specific subject (for example, a product like braised beef, as shown in \textbf{Example 2}, suddenly diverts attention to unrelated matters. After an extended exploration of these tangential topics, the narrative may return to the initial subject without explicitly reintroducing or reiterating the key terminologies or thematic markers associated with the original topic. Such interruptions and shifts can disrupt the cohesion and continuity of the discourse, posing significant challenges for natural language processing models tasked with long-context understanding. The absence of explicit referential cues upon returning to the original topic can lead to ambiguity, misinterpretation, and difficulties in maintaining a consistent thread of narrative, thereby complicating both the comprehension and summarization of the text.

% \begin{figure}
%     \centering
%         \includegraphics[width=1.0\linewidth]{figures/context_case_interruptions.pdf}
%     \caption{Cased of Topic Drift and Interruptions.}
%     \label{fig:interruptions}
% \end{figure}

   
% % $\bullet$~\textbf{Implicit and Incomplete References.} 
% $\bullet$~\textbf{Fragmented Discourse and Disconnected Semantic Links.} 
% The long-context in Live stream exhibit a highly fragmented discourse structure, characterized primarily by a lack of explicit logical connections and contextual cohesion among sentences (as illustrated in \textbf{Example 1}). These texts are composed of numerous independent, succinct sentences, each conveying a singular piece of information without the use of conventional cohesive devices or transitional markers typically present in more structured discourse. As a result, the relationships between these discrete informational units remain implicit and incomplete, necessitating that readers or automated models rely on background knowledge and additional inferential processes to reconstruct the overall context and fully comprehend the underlying meanings. This inherent fragmentation and the ensuing semantic gaps underscore the need for designing robust semantic understanding and inference mechanisms that can effectively address these implicit and incomplete dependencies. 
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/context_case_Implicit.pdf}
%     \caption{Case of Fragmented Discourse and Disconnected Semantic Links}
%     \label{fig:Fragmented}
% \end{figure}
\\
% $\bullet$~\textbf{High Redundancy and Repetitive Patterns.}

% In extended colloquial discourse, one frequently observes a substantial degree of redundancy and recurring expressions that provide minimal semantic contribution to the central narrative. As indicated by the word cloud in Figure~\ref{fig:Wordcloud}, phrases such as “what is it?”, “oh, my god.”, “it’s a shot.” and “it’s all right.” appear repeatedly and may recur at random intervals throughout the text. While such repetitions reflect the informal and spontaneous nature of spoken language, they can significantly impede a natural language processing model’s ability to maintain focus on core thematic elements. This high-frequency, low-information content inflates the overall text length and dilutes the signal-to-noise ratio, thereby complicating the identification of salient information. Moreover, these repetitive utterances risk overshadowing critical details or disrupting the coherence of the primary discourse thread. Consequently, it is imperative to develop robust text-processing strategies—encompassing filtering, summarization, and context-aware parsing—to effectively manage redundancy and repetition in large-scale colloquial corpora.
% $\bullet$~\textbf{Dispersed Key Information.}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/plot-length.pdf}
%     \caption{Distribution of the context length.}
%     \label{fig:enter-label}
% \end{figure}
% $\bullet$~\textbf{Diverse Context Length.} The dataset encompasses a wide range of context lengths, from short, focused interactions to extended, multi-turn exchanges. This diversity ensures that the dataset is suitable for testing models across varying levels of complexity, requiring them to adapt their strategies for both brief and long contexts.\textcolor{blue}{TODO:add the single,multi span here}

% $\bullet$~\textbf{Diverse Task Types.} To support comprehensive evaluation, the dataset is designed for multiple NLP tasks, including summarization, question answering, and relevance ranking. These tasks reflect common challenges in processing long texts and provide a basis for testing different aspects of a model performance, such as extracting key information, maintaining contextual coherence, and identifying relevant content.\textcolor{blue}{TODO:add the task types introduction here}


% $\bullet$~\textbf{Real Interactions Without Post-Processing.} The dataset captures natural interactions without heavy post-processing, preserving disfluencies, interruptions, and redundant expressions that occur in real-world conversations. This authenticity ensures that models are evaluated on realistic data, challenging them to handle the inherent imperfections of unstructured text effectively. \textcolor{blue}{TODO:add the some cases about the real interactions here}

% $\bullet$~\textbf{Rich Diversity in Topics and Domains.} The dataset covers a variety of topics and domains, ensuring a representative sample of real-world scenarios. This diversity enables the evaluation of models across a broad spectrum of content types, improving their generalizability to unseen data.

% Through these principles, our dataset not only serves as the first dataset in the domain of live interactions but also challenges and advances the understanding and processing capabilities of large models on long, redundancy-prone texts.



\subsection{Dataset Collection}
Based on the design principles outlined earlier, our dataset is constructed from Automatic Speech Recognition~(ASR) outputs of Live E-commerce. The data is collected, transcribed, and processed systematically to ensure it aligns with the requirements of long-text understanding tasks. Next, we will describe the data sources and the processing steps in detail.

\paragraph{Data Source.}
The data used in this study were collected from \textbf{Douyin} live streams, a widely recognized e-commerce streaming platform known for its diverse live streaming formats. To construct a representative dataset, we recorded and transcribed audio from e-commerce live sessions. These recordings encompass 11 major product categories and 32 subcategories, including apparel and lingerie, electronics, beauty and cosmetics, and household goods. These categories were carefully selected to encompass the diverse content and interaction styles characteristic of live-stream e-commerce, ensuring the dataset's broad applicability across multiple domains.

The selected live streams represent a variety of presentation styles, levels of audience engagement, and product types. Each session typically features a monologue by the host, real-time interactions with the audience, and multiparty discussions involving co-hosts or guest speakers. By capturing this diversity, the dataset reflects the authentic characteristics of spoken discourse in e-commerce live streams, such as promotional repetition, dynamic dialogues, and frequent audience-driven Q\&A exchanges. Figure~\ref{fig:domains} illustrates the distribution of the various e-commerce live stream categories included in the dataset.

\paragraph{Processing and Structuring.}
% ~\textcolor{blue}{ADD: license, data safety}
In this study, our raw video data is sourced exclusively from publicly accessible Douyin live streams, ensuring adherence to data safety and copyright regulations. The raw data exhibits a significant amount of redundancy and filler words, which poses challenges for rule-based processing methods; however, these characteristics are intrinsic to natural spoken language, where repetition often serves to emphasize key points. To extract the textual information from the audio, we employ a pre-trained speech-to-text model~\footnote{Whisper pre-trained on a large-scale audio corpus.} that preserves all repetitions and filler words, thereby maintaining the authenticity of the spoken context. After a thorough examination of the transcribed text, we implement a rigorous filtering strategy to remove meaningless elements typically introduced by background noise—specifically, instances where the same sentence appears consecutively more than ten times without contributing additional contextual value are pruned to enhance the overall quality of the dataset for subsequent analyses.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/case_retrieval_hybrid_v2.pdf}
    \caption{Cased of the retrieval and hybrid tasks.}
    \label{fig:case_retrieval_hybrid}
\end{figure}

\subsection{Task Construction}
To systematically evaluate large language models (LLMs) in processing and comprehending long-form textual data, we define three primary task categories, each differing in information granularity and cognitive demand: retrieval-dependent tasks, reasoning-dependent tasks, and hybrid tasks.

\paragraph{Retrieval-Dependent Tasks.}
These tasks require models to locate specific information from the text and provide direct answers, such as product prices, names, or specifications. This category focuses on the model’s capacity to identify and retrieve precise, relevant details from potentially extensive content. For instance, a model may be asked to determine the price of a particular product (Figure~\ref{fig:case_retrieval_hybrid}(a)) or verify whether an item qualifies for free shipping under a given logistics policy.

\paragraph{Reasoning-Dependent Tasks.}
These tasks extend beyond simple retrieval by requiring the model to infer or deduce answers through synthesizing information from the text, often supplemented by the model’s internal knowledge. Examples include identifying implicit product features, deducing promotional strategies, or classifying products by category in a live-stream transcript. Unlike retrieval-based tasks, these tasks necessitate establishing logical connections and deriving higher-level insights.

\paragraph{Hybrid Tasks.}
Hybrid tasks integrate both retrieval and reasoning requirements. Models must first retrieve multiple relevant pieces of information from the text, then perform reasoning to arrive at a coherent answer. A typical example involves comparing two products (\eg weight, battery life, or durability) based on details dispersed across different segments of the transcript (Figure~\ref{fig:case_retrieval_hybrid}(b)).

By categorizing tasks in this manner, we enable a comprehensive assessment of a model’s ability to process and interpret lengthy, detailed texts under varying degrees of complexity and cognitive demand.


% \section{Evaluation of KV Cache Compression}

